On $H^2$-gradient Flows for the Willmore Energy

We show that the concept of $H^2$-gradient flow for the Willmore energy and other functionals that depend at most quadratically on the second fundamental form is well-defined in the space of immersions of Sobolev class $W^{2,p}$ from a compact, $n$-dimensional manifold into Euclidean space, provided that $p \geq 2$ and $p>n$. We also discuss why this is not true for Sobolev class $H^2=W^{2,2}$. In the case of equality constraints, we provide sufficient conditions for the existence of the projected $H^2$-gradient flow and demonstrate its usability for optimization with several numerical examples.

==> ParabolicFlow.tex <==
\newpage

\section{Parabolic Flow}

Let $\cC=\Imm^{s,p}(\varSigma;\R^m)$ be a para-Riemannian manifold and let $F \colon \cC \to \R$ be a smooth morphism such that $\Hess(F)\at_f \colon \RX[\cC][f] \to \RY[\cC][f][\dual]$ is a compact perturbation of $\RJ[\cC]\at_f$, i.e., 
\begin{align*}
	\Hess(F)\at|_f = \RJ[\cC]\at_f + K\at_f
\end{align*}
with some symmetric compact operator $K \colon \RX[\cC] \to \RY[\cC][][\dual]$.

For $f \in C^0(I;\Imm^{s,p}(\varSigma;\R^m)) \cap W^{1,2}(I;L^2(\varSigma;\R^m))$, we consider the constraint parabolic flow defined by
\begin{align*}
	\pd_t f + DF(f) = 0, \qquad \varPhi(f(t)) = 0,
\end{align*}
in the sense that
\begin{align*}
	\int_{0}^T \!\!\!\int_\varSigma \ninnerprod{\pd_t f(x,t), w(x,t)} \, \vol_f\, \dd t + \int_{0}^T \!\! \ninnerprod{\RY[F][f(t)],w(t)} \, \dd t= 0
	\quad \text{for all $w \in C^\infty( I; C^\infty(\varSigma;\R^m)$}.
\end{align*}


\subsection{Time-discrete implicit Euler scheme}
Some scheme which resembles implicit Euler method:
\begin{align*}
	\left\{
	\begin{array}{rcl}
		M_{f_{i}} \left( \frac{f_{i+1}-f_{i}}{\tau} \right)
		+ \RY[F][f_{i+1}] &= &0, \\
		\varPhi(f_{i+1}) &= &0.
	\end{array}
	\right.
\end{align*}
With $f_{i+1} = \exp_{f_i} (u_i)$ and using Taylor's theorem:
\begin{align*}
	\left\{
	\begin{array}{rcl}
		M_{f_{i}} \, u_i 
		+ \tau\, \RY[F][f_{i}] + \tau\, \Hess(F)\at_{f_i} \, u_i
		&= 
		& \tau\, \LandO(\nnorm{u_i}_{W^{s,p}}^2), \\
		\varPhi(f_{i}) + \RX[\varPhi][f_i] \; u_i 
		&= 
		& \LandO(\nnorm{u_i}_{W^{s-\delta,p}}^2).
	\end{array}
	\right.
\end{align*}

Using $\Hess(F)\at_{f_i} = \RJ[E]\at_{f_i} + K\at_{f_i}$, we obtain
\begin{align*}
	\left\{
	\begin{array}{rcl}
		\big(
		\frac{1}{\tau} M_{f_{i}} + \RJ[\cC]\at_{f_i} \big)\, u_i
		&= 
		& - \RY[F][f_{i}] - K\at_{f_i} \, u_i + \LandO(\nnorm{u_i}_{W^{s,p}}^2), \\
		\RX[\varPhi][f_i] \; u_i 
		&= 
		& -\varPhi(f_{i}) + \LandO(\nnorm{u_i}_{W^{s-\delta,p}}^2).
	\end{array}
	\right.
\end{align*}
Know, we assume that 
\begin{align*}
	\nnorm{u_i}_{W^{s-\delta,p}}^2 \leq C\, \tau^2 
	\qand
	\nnorm{K\at_{f_i} \, (u_i -  u_{i-1})}_{\RY[\cC][f][\dual]}
	\leq C \,  \nnorm{u_i - u_{i-1}}_{W^{s-\eta,p}} \leq C\, \tau^2.
\end{align*}
Thus, upto $\Lando(\tau^2)$, this is the same as solving
\begin{align*}
	\left\{
	\begin{array}{rcl}
		\big(
		\frac{1}{\tau} M_{f_{i}} + \RJ[\cC]\at_{f_i} \big)\, u_i
		&= 
		& - \RY[F][f_{i}] - K\at_{f_i} \, u_{i-1}, \\
		\RX[\varPhi][f_i] \; u_i 
		&= 
		& -\varPhi(f_{i}).
	\end{array}
	\right.
\end{align*}
By introducing a Lagrange multiplier $\lambda_i$, we are lead to the saddle point system
\begin{align*}
	\begin{pmatrix}
		\frac{1}{\tau} M_{f_{i}} + \RJ[\cC]\at_{f_i}
		& \RY[\varPhi][f_i][\dual]\\
		\RX[\varPhi][f_i][\dual]
		&0
	\end{pmatrix}
	\begin{pmatrix}
		u_i \\ \lambda_i
	\end{pmatrix}	
	=
	\begin{pmatrix}
		- \RY[F][f_{i}] - K\at_{f_i} \, u_{i-1} \\ -\varPhi(f_{i})
	\end{pmatrix}.
\end{align*}

\begin{align*}
	\begin{pmatrix}
		M_{f_{i}} + \tau \, \RJ[\cC]\at_{f_i}
		& \RY[\varPhi][f_i][\dual]\\
		\RX[\varPhi][f_i][\dual]
		&0
	\end{pmatrix}
	\begin{pmatrix}
		u_i \\ \lambda_i
	\end{pmatrix}	
	=
	\begin{pmatrix}
		- \tau \, \RY[F][f_{i}] - \tau \, K\at_{f_i} \, u_{i-1} \\ -\varPhi(f_{i})
	\end{pmatrix}.
\end{align*}

Solving this equation is always uniquely possible for finite $\tau>0$. Connecting $(f_0,f_1,\dotsc,f_N)$ for $\tau = T/N$ by geodesics leads to a polygonal line $\gamma_N$ in $\cC$. 

A stability estimate is needed in order to show that the sequence $(\gamma_N)_{N\in \N}$ is suitabley bounded in $W^{1,p}(I; W^{s,p}(\varSigma;\R^m))$ such that weak convergence 
in $W^{1,p}(I; W^{s,p}(\varSigma;\R^m))$ and strong convergence in $C^0(I; W^{s,p}(\varSigma;\R^m))$ can be deduced.


\subsection{Time-continuous regularized scheme}

\begin{align*}
	\left\{
	\begin{array}{rcl}
		\bigparen{M_{f_\varepsilon(t)} + \varepsilon \, \RJ[\cC]\at_{f_\varepsilon(t)}} \,  \dot  f_\varepsilon(t)
		+ \RY[F][f_\varepsilon(t)] &= &0, \\
		\varPhi(f_\varepsilon(t)) &= &0.
	\end{array}
	\right.
\end{align*}
By introducing a Lagrange multiplier $\lambda(t)$, we are lead to the saddle point system
\begin{align*}
	\begin{pmatrix}
		\bigparen{M_{f_\varepsilon(t)} + \varepsilon \, \RJ[\cC]\at_{f_\varepsilon(t)}}
		& \RY[\varPhi][f_\varepsilon(t)][\dual]\\
		\RX[\varPhi][f_\varepsilon(t)][\dual]
		&0
	\end{pmatrix}
	\begin{pmatrix}
		\dot  f_\varepsilon(t) \\ \lambda(t)
	\end{pmatrix}	
	=
	\begin{pmatrix}
		- \RY[F][f_\varepsilon(t)] \\ -\varPhi(f_\varepsilon(t))
	\end{pmatrix}.
\end{align*}
Testing against $\Rj[\cC]\;\Ri[\cC]\;\dot f_\varepsilon(t)$ leads to
\begin{align*}
	\int_\varSigma \nabs{\dot f_\varepsilon(t)}^2 \, \vol_{f_\varepsilon(t)}
	+ \varepsilon \; \ninnerprod{
		\RJ[\cC]\at_{f_\varepsilon(t)}\; \dot f_\varepsilon(t), 
		\Rj[\cC]\;\Ri[\cC]\;\dot f_\varepsilon(t)
	}
	= - \tfrac{\dd}{\dd t} F(f_\varepsilon(t))
\end{align*}

\begin{align*}
	\int_\varSigma \nabs{\dot f_\varepsilon(t)}^2 \, \vol_{f_\varepsilon(t)}
	+ \varepsilon \; \ninnerprod{
		\RI[\cC]\at_{f_\varepsilon(t)}\; \Ri[\cC]\;\dot f_\varepsilon(t), 
		\Ri[\cC]\;\dot f_\varepsilon(t)
	}
	= - \tfrac{\dd}{\dd t} F(f_\varepsilon(t))
\end{align*}

\begin{align*}
	\int_0^T \!\!\int_\varSigma \nabs{\dot f_\varepsilon(t)}^2 \, \vol_{f_\varepsilon(t)} \, \dd t
	+ \varepsilon \; \int_0^T \!\!\ninnerprod{
		\RI[\cC]\at_{f_\varepsilon(t)}\; \Ri[\cC]\;\dot f_\varepsilon(t), 
		\Ri[\cC]\;\dot f_\varepsilon(t)
	}\, \dd t
	+ F(f_\varepsilon(T))
	= F(f_\varepsilon(0))
\end{align*}

Examples:
\begin{align*}
	\int_0^T \!\!\int_\varSigma \left(
		\nabs{\dot f_\varepsilon(t)}^2 
		+ \varepsilon \, \nabs{
			\dd \dot f_\varepsilon(t)
		}_{f_\varepsilon(t)}^2
		\right)\, \vol_{f_\varepsilon(t)} \, \dd t
	+ F(f_\varepsilon(T))
	= F(f_\varepsilon(0))
\end{align*}

\begin{align*}
	\int_0^T \!\!\int_\varSigma \left(
		\nabs{\dot f_\varepsilon(t)}^2 
		+ \varepsilon \, \nabs{
			\Delta_{f_\varepsilon(t)} \dot f_\varepsilon(t)
		}_{f_\varepsilon(t)}^2
		\right)\, \vol_{f_\varepsilon(t)} \, \dd t
	+ F(f_\varepsilon(T))
	= F(f_\varepsilon(0))
\end{align*}

Problem: How does the family of Riemannian metrics behave?
\begin{align*}
	g_\varepsilon(t)(X,Y) \ceq \ninnerprod{\dd f_\varepsilon(t)\,X, \dd f_\varepsilon(t)\,Y}_{\AmbSpace}
\end{align*}

\begin{align*}
	\frac{\dd}{\dd t}g_\varepsilon(t)(X,Y) 
	=
	\ninnerprod{\dd f_\varepsilon(t)\,X, \dd \dot f_\varepsilon(t)\,Y}_{\AmbSpace}
	+
	\ninnerprod{\dd \dot f_\varepsilon(t)\,X, \dd f_\varepsilon(t)\,Y}_{\AmbSpace}
\end{align*}

\section{Kato-Ponce Commutator Relations}

\emph{Ask Simon Blatt about it.}

\bigskip

Let $\cJ = (1-\Delta)^{\frac{1}{2}}$ be the Bessel potential and $s>0$.
For Schwartz functions $f$ and $g$, one has
\begin{align*}
	\nnorm{\cJ^s (f \cdot g) - f \cdot \cJ^s g}_{L^r}
	\leq C \, \left( 
		\nnorm{\dd f}_{L^{p_1}} \cdot \nnorm{\cJ^{s-1} g}_{L^{q_1}}
		+
		\nnorm{\cJ^s f}_{L^{p_2}} \cdot \nnorm{g}_{L^{q_2}}		
	\right)
\end{align*}
whenever $1< p_1,p_2,q_1,q_2 \leq \infty$, $1<r<\infty$, and $\frac{1}{r}=\frac{1}{p_1}+\frac{1}{q_1}=\frac{1}{p_2}+\frac{1}{q_2}$.

\bigskip

Some variants:

\bigskip

\emph{Original Kato-Ponce inequality}
\begin{align*}
	\nnorm{\cJ^s (f \cdot g) - f \cdot \cJ^s g}_{L^r}
	\leq C \, \left( 
		\nnorm{\cJ^1 f}_{L^{\infty}} \cdot \nnorm{\cJ^{s-1} g}_{L^{r}}
		+
		\nnorm{\cJ^s f}_{L^{r}} \cdot \nnorm{g}_{L^{\infty}}		
	\right)
\end{align*}

\emph{Fractional Leibniz rule}
\begin{align*}
	\nnorm{\cJ^s (f \cdot g)}_{L^r}
	\leq C \, \left( 
		\nnorm{f}_{L^{p_1}} \cdot \nnorm{\cJ^s g}_{L^{q_1}}
		+
		\nnorm{\cJ^s f}_{L^{p_2}} \cdot \nnorm{g}_{L^{q_2}}		
	\right)
\end{align*}

\emph{Kenig, Ponce, Vega}
$\cD = (-\Delta)^{\frac{1}{2}}$, $0<s,s_1,s_2<1$ with $s = s_1+s_2$, $1<r,p,q<\infty$
\begin{align*}
	\nnorm{\cD^s (f \cdot g) - f \cdot \cD^s g}_{L^r}
	\leq C \, \left( 
		\nnorm{\cD^{s_1} f}_{L^{p}} \cdot \nnorm{\cD^{s_2} g}_{L^{q}}
	\right)
\end{align*}

\section{Submanifold Constraints}

Let $\varphi \colon U\subset \AmbSpace \to \R^k$ be a submersion of class $C^\infty$ so that 
\begin{align*}
	M \ceq \set{y\in \AmbSpace | \varphi(x)=0}
\end{align*}
is a smooth submanifold. Thus $f \in W^{2,p}(\varSigma;M)$ can be encoded as
\begin{align*}
	f\in W^{2,p}(\varSigma;\AmbSpace)
	\quad
	\text{with}
	\varPhi(f) \ceq \varphi \circ f = 0.
\end{align*}
\begin{align*}
	H_M(f) = \Delta^M_f \, f = \pm (\nabla^{M,f})^*\dd = \dd^{*_f}\, (\pr(f) \, \dd f)
\end{align*}
\begin{align*}
	\nabla^{M,f}_X  \ceq \pr(f) \, \dd f\, X
\end{align*}
where $\pr(f)\at_x \ceq \id_{\AmbSpace} - (\dd \varphi\at_{f(x)})^\dagger(\dd \varphi\at_{f(x)}) \in \Hom(\AmbSpace;\AmbSpace)$ is the Euclidean orthoprojector onto $T_{f(x)}M = \ker (\dd \varphi\at_{f(x)})$.

The Willmore energy $\cW(f) \ceq \int_\varSigma \nabs{H_M(f)}^2 \, \vol_f$ and manifold constraint $\varPhi(f) \ceq \varphi \circ f$.
\begin{align*}
	\text{Minimize} \quad \cW(f) 
	\quad
	\text{subject to}
	\quad \varPhi(f) = 0.
\end{align*}

\section{Thoughts}

Let $f(x,t)$ satisfy
\begin{align*}
	\int \pd_t f(x,t) \, u + D\Willmore(f)\,u = 0
\end{align*}
\begin{align*}
	g(x,t) = f(\cdot, t)^\pull g_\AmbSpace\at_x = \pd_x f(x,t) \transp \pd_x f(x,t)
\end{align*}

\begin{align*}
	(M+ \tau \, L) \pd_t f = - \RY[\Willmore][f]
\end{align*}
\begin{align*}
	D_X (M+ \tau \, L) \pd_t f = - D_X \RY[\Willmore][f]
\end{align*}
\begin{align*}
	D_X \paren{(M+ \tau \, L) \pd_t f}
	= (M+ \tau \, L) \pd_t D_X f + \paren{D_X (M+ \tau \, L)} \pd_t f
	= - D_X \RY[\Willmore][f]
\end{align*}

\begin{align*}
	A_\tau(t) = M_{f_\tau(t)}+ \tau \, L_{f_\tau(t)}
\end{align*}
\begin{align*}
	A_\tau \pd_t D_X f 
	= - D_X \RY[\Willmore][f] + \paren{D_X A_\tau} \, A_\tau^{-1} \, \RY[\Willmore][f]
\end{align*}
\begin{align*}
	f_\tau(t + \tau) - f_\tau(t)
	= - A_\tau(t)^{-1}\RY[\Willmore][f_\tau(t)]
\end{align*}
\begin{align*}
	\paren{M_{f_\tau} + \tau \, L_{f_\tau}} \, \pd_t f_\tau = - \RY[\Willmore][f_\tau]
\end{align*}
Testing with $u = \pd_t f_\tau$.
\begin{align*}
	\int_{\varSigma \times I} \ninnerprod{\pd_t f_\tau, \pd_t f_\tau} \,\vol_{f_\tau} \, \dd t 
	+ \tau \, \int_{\varSigma \times I} \ninnerprod{\Delta_{f_\tau} \pd_t f_\tau,\Delta_{f_\tau} \pd_t f_\tau} \,\vol_{f_\tau} \, \dd t
	= - \int_{I} D\Willmore{f_\tau}\, \pd_t f_\tau \, \dd t
	= \Willmore(f_\tau(0)) - \Willmore(f_\tau(T))
\end{align*}
\begin{align*}
	\int_{\varSigma \times I} \nabs{\pd_t f_\tau}^2 \,\vol_{f_\tau} \, \dd t  
	+ \tau \, \int_{\varSigma \times I} \nabs{\Delta_{f_\tau} \pd_t f_\tau}^2 \,\vol_{f_\tau} \, \dd t    + \Willmore(f_\tau(T)) 
	= \Willmore(f(0))
\end{align*}


Testing with $u = f_\tau$.
\begin{align*}
	\int_{\varSigma \times I} \ninnerprod{\pd_t f_\tau, f_\tau} \,\vol_{f_\tau} \, \dd t 
	+ \tau \, \int_{\varSigma \times I} \ninnerprod{\Delta_{f_\tau} \pd_t f_\tau,\Delta_{f_\tau} f_\tau} \,\vol_{f_\tau} \, \dd t
	= - \int_I \RY[\Willmore][f_\tau] \, f_\tau \, \dd t
	= - (2+n- 4) \int_I  \Willmore(f_\tau) \, \dd t
\end{align*}
\begin{align*}
	\frac{\dd}{\dd t}\int_{\varSigma \times I} \nabs{f_\tau}^2 \,\vol_{f_\tau} \, \dd t  
	= \int_{\varSigma \times I} 2\ninnerprod{\pd_t f_\tau, f_\tau} \,\vol_{f_\tau} \, \dd t 
	+ \int_{\varSigma \times I} \nabs{f_\tau}^2 \, \ninnerprod{\dd f_\tau,\dd \pd_t f_\tau}\,\vol_{f_\tau} \, \dd t  
\end{align*}
\begin{align*}
	\frac{\dd}{\dd t}\int_{\varSigma \times I} \nabs{\Delta_{f_\tau} f_\tau}^2 \,\vol_{f_\tau} \, \dd t  
	= \int_{\varSigma \times I} 2\ninnerprod{\Delta_{f_\tau}\pd_t f_\tau, \Delta_{f_\tau}f_\tau} \,\vol_{f_\tau} \, \dd t 
	+ \int_{\varSigma \times I} \nabs{\Delta_{f_\tau} f_\tau}^2 \, \ninnerprod{\dd f_\tau,\dd \pd_t f_\tau}_{f_\tau}\,\vol_{f_\tau} \, \dd t  
\end{align*}

\begin{align*}
	\Willmore(f) = \int_\varSigma \nabs{\Delta_{f} f}^2 \, \vol_{f}
\end{align*}
\begin{align*}
	D\Willmore(f)\,u 
	= \int_\varSigma 2\, \ninnerprod{\Delta_{f} f,\Delta_{f} u} \, \vol_{f}
	+ \int_\varSigma 2 \ninnerprod{\Delta_{f} f, (D \Delta(f) \,u)\,f} \, \vol_{f}
	+ \int_\varSigma \nabs{\Delta_{f} f}^2 \, \ninnerprod{\dd f,\dd u}_f \, \vol_{f}
\end{align*}
\begin{align*}
	D\Willmore(f)\,f 
	&= (2+n) \Willmore(f)
	+ 2 \int_\varSigma \ninnerprod{\Delta_{f} f, (D \Delta(f) \,f)\,f} \, \vol_{f}
\end{align*}
$Dg(f) \, u = \dd f\transp \dd u + \dd u \transp \dd f$, hence
$Dg(f) \, f = 2 \, g(f)$.
\begin{align*}
	\Delta_f v = \det(\mathbf{g})^{-\frac{1}{2}} \pd_i \;\paren{ 
		\det(\mathbf{g})^{\frac{1}{2}} (\mathbf{g}^{-1})_{ij}
		} \;\pd_j v
\end{align*}
\begin{align*}
	(D\Delta(f)\, u)\,v 
	&= - \frac{1}{2}\det(\mathbf{g})^{-\frac{3}{2}}  (D\det)(\mathbf{g}) (D\mathbf{g}(f) \, u) \;\pd_i \;\paren{ 
		\det(\mathbf{g})^{\frac{1}{2}} (\mathbf{g}^{-1})_{ij}
		} \;\pd_j v
	\\
	&\qquad
	+ \frac{1}{2}  \det(\mathbf{g})^{-\frac{1}{2}} \pd_i \;\paren{ 
		\det(\mathbf{g})^{-\frac{1}{2}} \cdot
			\paren{
				(D\det)(\mathbf{g}) (D\mathbf{g}(f) \, u)
				} \cdot (\mathbf{g}^{-1})_{ij}
		} \;\pd_j v
	\\
	&\qquad
	- \det(\mathbf{g})^{-\frac{1}{2}} \pd_i \;\paren{ 
		\det(\mathbf{g})^{\frac{1}{2}} (\mathbf{g}^{-1} \cdot (D\mathbf{g}(f) \, u) \cdot \mathbf{g}^{-1})_{ij}
		} \;\pd_j v	
\end{align*}

\begin{align*}
	(D\det)(\mathbf{g}) (D\mathbf{g}(f) \, f)
	&= (D\det)(\mathbf{g}) (2 \, \mathbf{g})
	= \frac{\dd}{\dd s} \det(\mathbf{g} +2 \, s\mathbf{g} )\At_{s=0}
	\\
	&= \frac{\dd}{\dd s} \det(\mathbf{g}) (1+2 \, s)^n \At_{s=0}
	=  2\, n\, \det(\mathbf{g})
\end{align*}

\begin{align*}
	(D\Delta(f)\, f)\,v 
	&= - \frac{1}{2}\det(\mathbf{g})^{-\frac{3}{2}}  2\, n\, \det(\mathbf{g}) \;\pd_i \;\paren{ 
		\det(\mathbf{g})^{\frac{1}{2}} (\mathbf{g}^{-1})_{ij}
		} \;\pd_j v
	\\
	&\qquad
	+ \frac{1}{2}  \det(\mathbf{g})^{-\frac{1}{2}} \pd_i \;\paren{ 
		\det(\mathbf{g})^{-\frac{1}{2}} \cdot
		2\, n\, \det(\mathbf{g}) \cdot (\mathbf{g}^{-1})_{ij}
		} \;\pd_j v
	\\
	&\qquad
	- \det(\mathbf{g})^{-\frac{1}{2}} \pd_i \;\paren{ 
		\det(\mathbf{g})^{\frac{1}{2}} (\mathbf{g}^{-1} \cdot 2\, \mathbf{g} \cdot \mathbf{g}^{-1})_{ij}
		} \;\pd_j v	
	\\
	&= - n \, \det(\mathbf{g})^{-\frac{1}{2}}\;\pd_i \;\paren{ 
		\det(\mathbf{g})^{\frac{1}{2}} (\mathbf{g}^{-1})_{ij}
		} \;\pd_j v
	\\
	&\qquad
	+ n  \det(\mathbf{g})^{-\frac{1}{2}} \pd_i \;\paren{ 
		\det(\mathbf{g})^{\frac{1}{2}} \, (\mathbf{g}^{-1})_{ij}
		} \;\pd_j v
	\\
	&\qquad
	- 2 \, \det(\mathbf{g})^{-\frac{1}{2}} \pd_i \;\paren{ 
		\det(\mathbf{g})^{\frac{1}{2}} (\mathbf{g}^{-1})_{ij}
		} \;\pd_j v
	\\
	&= - 2 \, \Delta_f \, v				
\end{align*}
\begin{align*}
	D\Willmore(f)\,f 
	&= (2+n) \, \Willmore(f)
	+ 2 \int_\varSigma \ninnerprod{\Delta_{f} f, (D \Delta(f) \,f)\,f} \, \vol_{f}
	\\
	&= (2+n- 4) \, \Willmore(f)
\end{align*}



\newpage


\begin{align*}
	D \det(\mathbf{g})^{\frac{1}{2}}(f)\, u
	= \ninnerprod{\dd f, \dd u}_f \,  \det(\mathbf{g})^{\frac{1}{2}}
\end{align*}
\begin{align*}
	(D\Delta(f)\, u)\,v 
	&= - \frac{1}{2}\det(\mathbf{g})^{-\frac{3}{2}}  (D\det)(\mathbf{g}) (D\mathbf{g}(f) \, u) \;\pd_i \;\paren{ 
		\det(\mathbf{g})^{\frac{1}{2}} (\mathbf{g}^{-1})_{ij}
		} \;\pd_j v
	\\
	&\qquad
	+ \frac{1}{2}  \det(\mathbf{g})^{-\frac{1}{2}} \pd_i \;\paren{ 
		\ninnerprod{\dd f, \dd u}_f \, \det(\mathbf{g})^{\frac{1}{2}} \, (\mathbf{g}^{-1})_{ij}
		} \;\pd_j v
	\\
	&\qquad
	- \det(\mathbf{g})^{-\frac{1}{2}} \pd_i \;\paren{ 
		\det(\mathbf{g})^{\frac{1}{2}} (\mathbf{g}^{-1} \cdot (D\mathbf{g}(f) \, u) \cdot \mathbf{g}^{-1})_{ij}
		} \;\pd_j v	
\end{align*}x

\newpage
\begin{align*}
	f_\tau \in C^{1,1}(I; W^{2,p}(\varSigma;\AmbSpace)).
\end{align*}
\begin{align*}
	f \in C^0(I; W^{2,p}(\varSigma;\AmbSpace))
	\qquad
	\pd_t f \in L^p(I; (W^{2,p}(\varSigma;\AmbSpace))')
\end{align*}

\section{Hyperbolic Flow}

\begin{align*}
	\cL(f,\varrho) 
	&\ceq
	\frac{1}{2} \int_I \int_\varSigma \nabs{\dot f}^2 \, \varrho \, \vol_{f} \wedge \dd t
	- \int_I  \Willmore(f)\, \dd t
\end{align*}

\begin{align*}
	\ninnerprod{\dd \cL(f,\varrho) ,(u,\sigma)}
	&=
	\int_I \int_\varSigma 
	\paren{
		\ninnerprod{\dot  f,\dot  u} \, \varrho 
		+ \nabs{\dot  f}^2 \, \ninnerprod{\dd f,\dd u}_{f} \, \varrho
		+ \nabs{\dot  f}^2 \, \sigma
	}\, \vol_{f} \wedge \dd t
	- \int_I  \ninnerprod{\dd \Willmore\at_{f}, u}\, \dd t
	\\
	&=
	\int_I \int_\varSigma 
	\paren{
		\ninnerprod{\dot f,\dot u}
		+ \nabs{\dot f}^2 \, \ninnerprod{\dd f,\dd u}_{f}
		+ \nabs{\dot f}^2 \, \tfrac{\sigma}{\varrho}
	}\, \varrho\, \vol_{f} \wedge \dd t
	- \int_I  \ninnerprod{\dd \Willmore\at_{f}, u}\, \dd t
\end{align*}
\begin{align*}
	\varPhi(f,\varrho) &\ceq \varrho \, \vol_{f} - \vol_\ReferenceMetric
\end{align*}
\begin{align*}
	\Manifold \ceq \set{(f,\varrho) \in \Imm^{2,p}(\varSigma;\AmbSpace) \times W^{1,p}(\varSigma;\R_+)
		|
		\varPhi(f,\varrho) = 0
	}
\end{align*}
\begin{align*}
	T_{(f,\varrho)}\varPhi\,(u,\sigma) 
	&= \sigma \, \vol_{f} + \varrho \, \ninnerprod{\dd f,\dd u}_{f} \, \vol_{f}
	= \paren{ \tfrac{\sigma}{\varrho} + \ninnerprod{\dd f,\dd u}_{f}} \, \vol_{g_0}
\end{align*}

For a curve $(f,\varrho) \colon I \to \cM$ and a vector field $(u,\sigma)$ along $(f,\varrho)$ and tangent to $\cM$, we obtain
\begin{align*}
	\ninnerprod{\dd \cL(f,\varrho) ,(u,\sigma)}
	&=
	\int_I \int_\varSigma 
		\ninnerprod{\dot f,\dot u}
	\, \vol_\ReferenceMetric \wedge \dd t
	- \int_I  \ninnerprod{\dd \Willmore\at_{f}, u}\, \dd t
	= 0
\end{align*}


\begin{align*}
	\int_I \int_\varSigma 
		\ninnerprod{\dot f,\dot u}
	\, \vol_\ReferenceMetric \, \dd t
	+
	\tau
	\int_I
	\int_\varSigma 
		\ninnerprod{\Delta_f\, \dot f,\Delta_f \, \dot u}
	\, \vol_{f(t)}\, \dd t
	=
	\int_I \ninnerprod{\dd \Willmore\at_{f}, u}\, \dd t
\end{align*}

Integration by parts (in time):
\begin{align*}
	-\int_I \int_\varSigma 
		\ninnerprod{\ddot f,u}
	\, \vol_\ReferenceMetric \, \dd t
	-
	\tau
	\int_I
	G_f \paren{\tfrac{\nabla}{\dd t} \dot f,u} \, \dd t
	=
	\int_I \ninnerprod{\dd \Willmore\at_{f}, u}\, \dd t
\end{align*}
\begin{align*}
	\tfrac{\nabla}{\dd t} \dot f = \ddot f + \varGamma_{\dot f} \dot f
\end{align*}
\begin{align*}
	M_f \, \ddot f + \tau \, L_f \, \tfrac{\nabla}{\dd t} \dot f = - \RY[\Willmore][f]
\end{align*}

\begin{align*}
	(M_f  + \tau \, L_f) \, \ddot f = - \RY[\Willmore][f] - \tau \, L_f \, \varGamma_{\dot f} \dot f
\end{align*}
\begin{align*}
	v \ceq \dot f
\end{align*}
\begin{align*}
	\begin{pmatrix}
		(M_f  + \tau \, L_f) &0
		\\
		1 & -1
	\end{pmatrix}
	\begin{pmatrix}
		\dot v \\ \dot f
	\end{pmatrix}
	=
	\begin{pmatrix}
		- \RY[\Willmore][f] - \tau \, L_f \, \varGamma_{\dot f} \dot f \\ 0
	\end{pmatrix}	
\end{align*}

\newpage

\subsection{Easier alternative}
\begin{align*}
	\int_I \int_\varSigma \paren{
		\ninnerprod{\dot f,\dot u} 
		+
		\tau \ninnerprod{\Delta_\ReferenceMetric\, \dot f,\Delta_\ReferenceMetric \, \dot u}
	}\, \vol_\ReferenceMetric\, \dd t
	=
	\int_I \ninnerprod{\dd \Willmore\at_{f}, u}\, \dd t
\end{align*}

Integration by parts in time:
\begin{align*}
	\int_I \int_\varSigma \paren{
		\ninnerprod{\ddot f,u} 
		+
		\tau \ninnerprod{\Delta_\ReferenceMetric\, \ddot f,\Delta_\ReferenceMetric \, u}
	}\, \vol_\ReferenceMetric\, \dd t
	=
	-\int_I \ninnerprod{\dd \Willmore\at_{f}, u}\, \dd t
\end{align*}
Fundamental lemma:
\begin{align*}
	(M + \tau L)\, \ddot f + \RY[\varPhi][f][\dual] \, \lambda = - \RY[\Willmore][f] 
	\qand
	\RX[\varPhi][f]\, \dot f = 0
\end{align*}

\begin{align*}
	\begin{pmatrix}
		(M  + \tau \, L) &0 &\RY[\varPhi][f][\dual]
		\\
		 & 1 &0
		\\
		0 & \RX[\varPhi][f] &0 
	\end{pmatrix}
	\begin{pmatrix}
		\dot v \\ \dot f \\ \lambda
	\end{pmatrix}
	=
	\begin{pmatrix}
		- \RY[\Willmore][f]  \\ v \\ 0
	\end{pmatrix}	
\end{align*}

\subsection{Time-Discrete Equations}

We use PL ansatz functions in time for $f$ and $u$:
\begin{align*}
	\ddot f = (f_{i+1} - f_i)/\delta t 
	\qand
	\ddot u = (u_{i+1} - u_i)/\delta t 	
\end{align*}
\begin{align*}
	f_{i+1} = f_i + \delta t \, v_i	
\end{align*}
\begin{align*}
	u_{i+1} = w, \qand u_i = 0.
\end{align*}
\begin{align*}
	\int_\varSigma 
		\ninnerprod{v_i,w}
	\, \vol_\ReferenceMetric \, \delta t
	+
	\tau
	\int_\varSigma 
		\ninnerprod{\Delta_{f_i}\, v_i,\Delta_{f_i} \,w}
	\, \vol_{f_i}\, \delta t
	=
	\frac{1}{2}
	\paren{
		\ninnerprod{\dd \Willmore\at_{f_{i+1}}, w}
	} \,	
	\delta t
\end{align*}

==> Subspaces.tex <==
\section{Subspaces}

\begin{proposition}\label{prop:subspace}
Let be a \UnnamedSpace $E_2$.
Let $\RX[E_1] \subset \RX[E_2]$ be a closed subspace and put $\RH[E_1] \ceq \overline{\Ri[E_2](\RX[E_1])}$ and $\RY[E_1] \ceq \overline{\Rj[E_2](\RY[E_1])}$. 
Then there are unique continuous, dense injections $\Ri[E_1] \colon \RX[E_1] \hookrightarrow \RH[E_1]$ and $\Rj[E_1] \colon \RH[E_1] \hookrightarrow \RY[E_1]$ such that the following diagram commutes.
\begin{equation*}
\begin{tikzcd}[]
	\RX[E_1] \ar[rr,hook] \ar[d,hook, two heads,"{\Ri[E_1]}"']
	&
	& \RX[E_2] \ar[d,hook, two heads,"{\Ri[E_2]}"]
	\\
	\RH[E_1] \ar[rr,hook] \ar[d,hook, two heads,"{\Rj[E_1]}"']
	&
	& \RH[E_2] \ar[d,hook, two heads,"{\Rj[E_2]}"]
	\\
	\RY[E_1] \ar[rr,hook] 
	&
	& \RY[E_2]\nospaceperiod
\end{tikzcd}
\end{equation*}
The space $\RH[E_1]$ equipped with the inherited inner product given by 
\begin{align*}
	\ninnerprod{v_1,v_2}_{\RH[E_1]} \ceq \ninnerprod{v_1,v_2}_{\RH[E_2]} 
	\quad \text{for $v_1$, $v_2 \in \RH[E_1]$}
\end{align*}
is in a natural way a Hilbert space.

The continuous linear operator $\RJ[E_1] \colon \RX[E_1] \to \RY[E_1][][\dual]$ defined by
\begin{align*}
	\ninnerprod{\RJ[E_1] \, u, w} \ceq \ninnerprod{\RJ[E_2] \,  u, w}
	\quad
	\text{for $u \in \RX[E_1]$, $w \in \RY[E_1]$}
\end{align*}
satisfies
\begin{enumerate}
	\item $\Rj[E_1]\dual \; \RJ[E_1] = \RI[E_1] \; \Ri[E_1]$.
	\item $\RJ[E_1]$ is injective.
	\item If $\RY[E_1]$ is reflexive then $\ima(\RJ[E_1]) \subset \RY[E_1][][\dual]$ is dense.	
\end{enumerate}
Thus $E_1$ equipped with $(\Ri[E_1],\Rj[E_1],\RI[E_1],\RJ[E_1])$ is a \UnnamedSpace if and only if $\RJ[E_1]$ is surjective.
\end{proposition}
\begin{proof}
\textbf{Claim 1:} Denote the canonical inclusion of $\RZ[E_1]$ into $\RZ[E_2]$ by $\RZ[A]$ for $\RZ \in \{\RX,\RH,\RY\}$.
Now the claim is readily verified by
\begin{align*}
	\ninnerprod{\Rj[E_1]\dual \; \RJ[E_1] \, u, v}  = \ninnerprod{\RJ[E_1] \, u, \Rj[E_1] \; v} 
	&= \ninnerprod{\RJ[E_2] \; \RX[A] \;  u, \RY[A] \; \Rj[E_1] \; v}
	 = \ninnerprod{\RJ[E_2] \; \RX[A] \;  u, \Rj[E_2] \; \RY[A] \;  v}	
	\\	
	&= \ninnerprod{\RI[E_2] \; \Ri[E_2] \; \RX[A] \;  u, \RY[A] \;  v}		
	 = \ninnerprod{\RI[E_2] \; \RX[A] \;  \Ri[E_1] \; u, \RY[A] \;  v}			
	\\	
	&= \ninnerprod{\RI[E_2] \; \RX[A] \;  \Ri[E_1] \; u, \RY[A] \;  v}				
	 = \ninnerprod{\RI[E_1] \; \Ri[E_1] \; u, v}.
\end{align*}
\newline
\textbf{Claim 2:} 
For each $u \in \RX[E_1] \setminus\{0\}$, we have $\ninnerprod{\RJ[E_1] \; u ,\Rj[E_1] \; \Ri[E_1] \; u} = \ninnerprod{\Ri[E_1] \; u ,\Ri[E_1] \; u}_{\RH[E_1]} >0$, thus $\RJ[E_1]$ is injective.
\newline
\textbf{Claim 3:} \emph{Assume} there is $\psi \in \RY[E_1][][\dual]\setminus \overline{\ima(\RJ[E_1])}$. Since $\RY[E_1]$ is reflexive, there is a $w \in \RY[E_1]$ with $\ninnerprod{\psi,w} \neq 0$ and $\ninnerprod{\RJ[E_1] \, u ,w} = 0$ for all $u \in \RX[E_1]$ (Hahn-Banach theorem).
Since $\Rj[E_1] \, \Ri[E_1](\RX[E_1]) \subset \RY[E_1]$ is dense, we find a sequence $u_n \in \RX[E_1]$ with $w = \lim_{n \to \infty} \Rj[E_1] \, \Ri[E_1] \, u_n$.
This leads inevitably to the \emph{contradiction}
$
	\ninnerprod{\RJ[E_1]\;u , w}
	= \lim_{n\to\infty}\ninnerprod{\RJ[E_1]\;u , \Rj[E_1]\;\Ri[E_1]\; u_n} = 0.
$
Hence $\ima(\RJ[E_1]) \subset \RY[E_1][][\dual]$ is dense. 
\end{proof}
\fxnote{Why cannot we expect $J$ to be invertible in general?}

\newpage


\begin{proposition}\label{prop:subspace1}
Let be a \UnnamedSpace $E_1$ and let $E_0 \subset E_1$ be a split subspace with projector $P \in \RMor(E_1;E_1)$. Denote by $\Ri[E_0] \colon \RX[E_0] \to \RH[E_0]$ and $\Rj[E_0] \colon \RH[E_0] \to \RY[E_0]$ the canonical injections induced by $\Ri[E_1]$ and $\Rj[E_1]$, respectively; and by $A=(\RX[A],\RH[A],\RY[A]) \colon E_0 \hookrightarrow E_1$ the canonical injection.
\begin{align*}
	\RI[E_0] \ceq \RH[A][][\dual] \; \RI[E_1] \; \RH[A]
	\qand
	\RJ[E_0] \ceq \RY[A][][\dual] \; \RJ[E_1] \; \RX[A]	
\end{align*}
\end{proposition}
\begin{align*}
	\RJ[E_0] \ceq \RY[A][][\dual] \; \RJ[E_1] \; \RX[A]	
\end{align*}

\begin{align*}
	L \ceq \RX[B][][] \; \RJ[E_1]^{-1} \; \RY[B][][\dual]
\end{align*}
\begin{align*}
	L \; \RJ[E_0]  = \RX[B][][] \; \RJ[E_1]^{-1} \; \RY[(A\,B)][][\dual] \; \RJ[E_1] \; \RX[A]	
	= \RX[B][][] \; \RJ[E_1]^{-1} \; \RY[P][][\dual] \; \RJ[E_1] \; \RX[A]	
\end{align*}

\begin{align*}
	\RJ[E_1] =
	\RJ[E_1] \, \RX[P] + \RJ[E_1] \, (1-\RX[P])
\end{align*}
\begin{align*}
	\RX[Q] \ceq \RJ[E_1]^{-1} \; \RY[P][][\dual] \; \RJ[E_1],
	\quad
	\RH[Q] \ceq \RI[E_1]^{-1} \; \RH[P][][\dual] \; \RI[E_1] ,
	\quad
	\RY[Q] \ceq \RK[E_1]^{-1} \; \RY[P][][\dual] \; \RK[E_1]
\end{align*}
